Olmo 3

We introduce Olmo 3, a family of state-of-the-art, fully-open language models at the 7B and 32B parameter scales. Olmo 3 model construction targets long-context reasoning, function calling, coding, instruction following, general chat, and knowledge recall. This release includes the entire model flow, i.e., the full lifecycle of the family of models, including every stage, checkpoint, data point, and dependency used to build it. Our flagship model, Olmo 3 Think 32B, is the strongest fully-open thinking model released to-date.

==> ai2style/defns.tex <==
%
% A useful set of commands
\usepackage{mathtools}
\usepackage{dsfont}
\usepackage[dvipsnames]{xcolor}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage{booktabs}
\usepackage{xfrac}
\usepackage{bbm}

\usepackage{algpseudocode}
\usepackage{algorithm}
\usepackage{algorithmicx}

\usepackage[most]{tcolorbox}
\usepackage{xparse}
\usepackage{lipsum}
\usepackage{changepage}
\usepackage{enumitem}

\newcommand{\qedwhite}{\hfill \ensuremath{\Box}}

%http://www-db.stanford.edu/~manku/latex.html
%The itemize environment can be replaced by:
\newcommand{\squishlist}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{3pt}
      \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishlisttwo}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}    \setlength{\parsep}{0pt}
      \setlength{\topsep}{0pt}     \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{2em} \setlength{\labelwidth}{1.5em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishend}{
    \end{list}  }

%Example usage: \squishlist    %% \begin{itemize}
%\item First item
%\item Second item
%\squishend     %% \end{itemize}

\newcommand{\denselist}{\itemsep 0pt\topsep-6pt\partopsep-6pt}


\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}{Corollary}[section]
\newtheorem{defn}{Definition}[section]
\newenvironment{mythm}{{\bf Theorem}}{}



\newcommand{\tm}{\tilde{m}}
\newcommand{\tv}{\tilde{v}}

% For bold vector symbols
\newcommand{\myvec}[1]{\boldsymbol{#1}}
\newcommand{\myvecsym}[1]{\boldsymbol{#1}}
\newcommand{\ind}[1]{\mathbb{I}(#1)}

\newcommand{\vzero}{\myvecsym{0}}
\newcommand{\vone}{\myvecsym{1}}
\newcommand{\valpha}{\myvecsym{\alpha}}
\newcommand{\vbeta}{\myvecsym{\beta}}
\newcommand{\vchi}{\myvecsym{\chi}}
\newcommand{\vdelta}{\myvecsym{\delta}}
\newcommand{\vDelta}{\myvecsym{\Delta}}
\newcommand{\vepsilon}{\myvecsym{\epsilon}}
\newcommand{\vell}{\myvecsym{\ell}}
\newcommand{\veta}{\myvecsym{\eta}}
\newcommand{\vgamma}{\myvecsym{\gamma}}
\newcommand{\vGamma}{\myvecsym{\Gamma}}
\newcommand{\vmu}{\myvecsym{\mu}}
\newcommand{\vnu}{\myvecsym{\nu}}
\newcommand{\vkappa}{\myvecsym{\kappa}}
\newcommand{\vlambda}{\myvecsym{\lambda}}
\newcommand{\vLambda}{\myvecsym{\Lambda}}
\newcommand{\vLambdaBar}{\overline{\vLambda}}
\newcommand{\vomega}{\myvecsym{\omega}}
\newcommand{\vOmega}{\myvecsym{\Omega}}
\newcommand{\vphi}{\myvecsym{\phi}}
\newcommand{\vPhi}{\myvecsym{\Phi}}
\newcommand{\vpi}{\myvecsym{\pi}}
\newcommand{\vpsi}{\myvecsym{\psi}}
\newcommand{\vPsi}{\myvecsym{\Psi}}
\newcommand{\vtheta}{\myvecsym{\theta}}
\newcommand{\vTheta}{\myvecsym{\Theta}}
\newcommand{\vsigma}{\myvecsym{\sigma}}
\newcommand{\vSigma}{\myvecsym{\Sigma}}
\newcommand{\vtau}{\myvecsym{\tau}}
\newcommand{\vupsilon}{\myvecsym{\upsilon}}
\newcommand{\vxi}{\myvecsym{\xi}}

\newcommand{\vxn}{\vx^{(n)}}

\newcommand{\vmuY}{\vb}
\newcommand{\vmuMu}{\vmu_{x}}
\newcommand{\vmuMuGivenY}{\vmu_{x|y}}
\newcommand{\vSigmaMu}{\vSigma_{x}}
\newcommand{\vSigmaMuInv}{\vSigma_{x}^{-1}}
\newcommand{\vSigmaMuGivenY}{\vSigma_{x|y}}
\newcommand{\vSigmaMuGivenYinv}{\vSigma_{x|y}^{-1}}
\newcommand{\vSigmaY}{\vSigma_{y}}
\newcommand{\vSigmaYinv}{\vSigma_{y}^{-1}}

%\newcommand{\vmuY}{\vmu_{y}}
%\newcommand{\vmuMu}{\vmu_{\mu}}
%\newcommand{\vmuMuGivenY}{\vmu_{\mu|y}}
%\newcommand{\vSigmaMu}{\vSigma_{\mu}}
%\newcommand{\vSigmaMuInv}{\vSigma_{\mu}^{-1}}
%\newcommand{\vSigmaMuGivenY}{\vSigma_{\mu|y}}
%\newcommand{\vSigmaMuGivenYinv}{\vSigma_{\mu|y}^{-1}}
%\newcommand{\vSigmaY}{\vSigma_{y}}
%\newcommand{\vSigmaYinv}{\vSigma_{y}^{-1}}

\newcommand{\muY}{\mu_{y}}
\newcommand{\muMu}{\mu_{\mu}}
\newcommand{\muMuGivenY}{\mu_{\mu|y}}
\newcommand{\SigmaMu}{\Sigma_{\mu}}
\newcommand{\SigmaMuInv}{\Sigma_{\mu}^{-1}}
\newcommand{\SigmaMuGivenY}{\Sigma_{\mu|y}}
\newcommand{\SigmaMuGivenYinv}{\Sigma_{\mu|y}^{-1}}
\newcommand{\SigmaY}{\Sigma_{y}}
\newcommand{\SigmaYinv}{\Sigma_{y}^{-1}}

\newcommand{\hatf}{\hat{f}}
\newcommand{\haty}{\hat{y}}
\newcommand{\const}{\mbox{const}}
\newcommand{\sigmoid}{\mbox{sigm}}

\newcommand{\one}{(1)}
\newcommand{\two}{(2)}

\newcommand{\va}{\myvec{a}}
\newcommand{\vb}{\myvec{b}}
\newcommand{\vc}{\myvec{c}}
\newcommand{\vd}{\myvec{d}}
\newcommand{\ve}{\myvec{e}}
\newcommand{\vf}{\myvec{f}}
\newcommand{\vg}{\myvec{g}}
\newcommand{\vh}{\myvec{h}}
\newcommand{\vj}{\myvec{j}}
\newcommand{\vk}{\myvec{k}}
\newcommand{\vl}{\myvec{l}}
\newcommand{\vm}{\myvec{m}}
\newcommand{\vn}{\myvec{n}}
\newcommand{\vo}{\myvec{o}}
\newcommand{\vp}{\myvec{p}}
\newcommand{\vq}{\myvec{q}}
\newcommand{\vr}{\myvec{r}}
\newcommand{\vs}{\myvec{s}}
\newcommand{\vt}{\myvec{t}}
\newcommand{\vu}{\myvec{u}}
\newcommand{\vv}{\myvec{v}}
\newcommand{\vw}{\myvec{w}}
\newcommand{\vws}{\vw_s}
\newcommand{\vwh}{\hat{\vw}}
\newcommand{\vx}{\myvec{x}}
%\newcommand{\vx}{\myvec{x}}
\newcommand{\vxt}{\myvec{\tilde{x}}}
\newcommand{\vy}{\myvec{y}}
\newcommand{\vyt}{\myvec{\tilde{y}}}
\newcommand{\vz}{\myvec{z}}

\newcommand{\vA}{\myvec{A}}
\newcommand{\vB}{\myvec{B}}
\newcommand{\vC}{\myvec{C}}
\newcommand{\vD}{\myvec{D}}
\newcommand{\vE}{\myvec{E}}
\newcommand{\vF}{\myvec{F}}
\newcommand{\vG}{\myvec{G}}
\newcommand{\vH}{\myvec{H}}
\newcommand{\vI}{\myvec{I}}
\newcommand{\vJ}{\myvec{J}}
\newcommand{\vK}{\myvec{K}}
\newcommand{\vL}{\myvec{L}}
\newcommand{\vM}{\myvec{M}}
\newcommand{\vN}{\myvec{N}}
\newcommand{\vO}{\myvec{O}}
\newcommand{\vP}{\myvec{P}}
\newcommand{\vQ}{\myvec{Q}}
\newcommand{\vR}{\myvec{R}}
\newcommand{\vS}{\myvec{S}}
\newcommand{\vT}{\myvec{T}}
\newcommand{\vU}{\myvec{U}}
\newcommand{\vV}{\myvec{V}}
\newcommand{\vW}{\myvec{W}}
\newcommand{\vX}{\myvec{X}}
%\newcommand{\vXs}{\vX_{\vs}}
\newcommand{\vXs}{\vX_{s}}
\newcommand{\vXt}{\myvec{\tilde{X}}}
\newcommand{\vY}{\myvec{Y}}
\newcommand{\vZ}{\myvec{Z}}


\newcommand{\vxtest}{\myvec{x}_*}
\newcommand{\vytest}{\myvec{y}_*}


\newcommand{\ftrue}{f_{true}}

\newcommand{\myprec}{\mbox{prec}}
\newcommand{\precw}{\lambda_{w}} % precision of weights (alpha)
\newcommand{\precy}{\lambda_{y}} % precision of y (beta)
\newcommand{\fbar}{\overline{f}}
\newcommand{\xmybar}{\overline{x}}
\newcommand{\ybar}{\overline{y}}
\newcommand{\zbar}{\overline{z}}
\newcommand{\vxbar}{\overline{\vx}}
\newcommand{\vXbar}{\overline{\vX}}
\newcommand{\vybar}{\overline{\vy}}
\newcommand{\vYbar}{\overline{\vY}}
\newcommand{\vzbar}{\overline{\vz}}
\newcommand{\vZbar}{\overline{\vZ}}
\newcommand{\xbar}{\overline{x}}
\newcommand{\Xbar}{\overline{X}}
\newcommand{\Ybar}{\overline{Y}}
\newcommand{\Gbar}{\overline{G}}
\newcommand{\Jbar}{\overline{J}}
\newcommand{\Lbar}{\overline{L}}
\newcommand{\Nbar}{\overline{N}}
%\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Tbar}{\overline{T}}
\newcommand{\Sbar}{\overline{S}}
\newcommand{\vSbar}{\overline{\vS}}
\newcommand{\Rbar}{\overline{R}}

\newcommand{\vtaubar}{\overline{\vtau}}
\newcommand{\vtbar}{\overline{\vt}}
\newcommand{\vsbar}{\overline{\vs}}

\newcommand{\htilde}{\tilde{h}}
\newcommand{\vhtilde}{\tilde{\vh}}
\newcommand{\Dtilde}{\tilde{D}}
\newcommand{\Ftilde}{\tilde{F}}
\newcommand{\wtilde}{\tilde{w}}
\newcommand{\ptilde}{\tilde{p}}
\newcommand{\pemp}{p_{emp}}
\newcommand{\pstar}{p^*}
\newcommand{\xtilde}{\tilde{x}}
\newcommand{\Xtilde}{\tilde{X}}
\newcommand{\ytilde}{\tilde{y}}
\newcommand{\Ytilde}{\tilde{Y}}
\newcommand{\vxtilde}{\tilde{\vx}}
\newcommand{\vytilde}{\tilde{\vy}}
\newcommand{\ztilde}{\tilde{\z}}
\newcommand{\vztilde}{\tilde{\vz}}
\newcommand{\vthetaMAP}{\hat{\vtheta}_{MAP}}
\newcommand{\vthetaS}{\vtheta^{(s)}}
\newcommand{\vthetahat}{\hat{\vtheta}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\overline{\theta}}
\newcommand{\vthetabar}{\overline{\vtheta}}
\newcommand{\pibar}{\overline{\pi}}
\newcommand{\vpibar}{\overline{\vpi}}


%\newcommand{\subsubsubsection}[1]{\paragraph{#1}}
\newcommand{\choice}[2]{\left(\!\!\! \begin{array}{c} #1 \\ #2\end{array} \!\!\!\right)}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\defeq}{\stackrel{\rm def}{=}}
\newcommand{\real}{\mathbb{R}}

\newcommand{\given}{\|}
\newcommand{\indep}[2]{{#1} \perp {#2}}
\newcommand{\condindep}[3]{{#1} \perp {#2} | {#3}}
\newcommand{\condindepG}[3]{{#1} \perp_G {#2} | {#3}}
\newcommand{\condindepP}[3]{{#1} \perp_p {#2} | {#3}}
\newcommand{\depend}[2]{{#1} \not \perp {#2}}
\newcommand{\conddepend}[3]{{#1} \not \perp {#2} | {#3}}

\newcommand{\trans}[1]{{#1}^{\mathtt{T}}}
\newcommand{\inv}[1]{{#1}^{-1}}

\newcommand{\ra}{\rightarrow}
\newcommand{\lra}{\leftrightarrow}
\newcommand{\Ra}{\Rightarrow}
%\newcommand{\rv}{r.v.}
\newcommand{\la}{\leftarrow}
\newcommand{\tr}{\mbox{tr}}
\newcommand{\st}{\mbox{  s.t.  }}

\newcommand{\dom}{\mbox{dom}}
\newcommand{\bel}{\mbox{bel}}
\newcommand{\dsep}{\mbox{dsep}}
\newcommand{\sep}{\mbox{sep}}
\newcommand{\entails}{\models}
\newcommand{\range}{\mbox{range}}
\newcommand{\myspan}{\mbox{span}}
\newcommand{\nullspace}{\mbox{nullspace}}
\newcommand{\adj}{\mbox{adj}}

\newcommand{\nbd}{\mbox{nbd}}
\newcommand{\nbr}{\mbox{nbr}}
\newcommand{\anc}{\mbox{anc}}
\newcommand{\desc}{\mbox{desc}}
\newcommand{\pred}{\mbox{pred}}
\newcommand{\nondesc}{\mbox{nondesc}}
\newcommand{\pa}{\pi}
\newcommand{\ch}{\mbox{ch}}
\newcommand{\mb}{\mbox{mb}}
\newcommand{\connects}{\sim}


\newcommand{\betadist}{\mbox{Beta}}
\newcommand{\Betadist}{\mbox{Beta}}
\newcommand{\bernoulli}{\mbox{Ber}}
\newcommand{\Ber}{\mbox{Ber}}
\newcommand{\Binom}{\mbox{Bin}}
\newcommand{\NegBinom}{\mbox{NegBinom}}
\newcommand{\binomdist}{\mbox{Bin}}
\newcommand{\cauchy}{\mbox{Cauchy}}
\newcommand{\DE}{\mbox{DE}}
\newcommand{\Dir}{\mbox{Dir}}
\newcommand{\discrete}{\calM}
\newcommand{\Discrete}{\calM}
\newcommand{\expdist}{\mbox{Exp}}
\newcommand{\expon}{\mbox{Expon}}
\newcommand{\gammadist}{\mbox{Ga}}
\newcommand{\Ga}{\mbox{Ga}}
\newcommand{\gauss}{{\cal N}}
\newcommand{\IG}{\mbox{IG}}
\newcommand{\IGauss}{\mbox{InvGauss}}
\newcommand{\IW}{\mbox{IW}}
\newcommand{\Laplace}{\mbox{Lap}}
\newcommand{\Mu}{\mbox{Mu}}
\newcommand{\Multi}{\mbox{Mu}}
\newcommand{\NIX}{NI\chi^2}
\newcommand{\GIX}{NI\chi^2}
\newcommand{\NIG}{\mbox{NIG}}
\newcommand{\GIG}{\mbox{NIG}}
\newcommand{\NIW}{\mbox{NIW}}
\newcommand{\GIW}{\mbox{NIW}}
\newcommand{\MVNIW}{\mbox{NIW}}
\newcommand{\NW}{\mbox{NWi}}
\newcommand{\MVNIG}{\mbox{NIG}}
\newcommand{\NGdist}{\mbox{NG}}
\newcommand{\prob}{p}
\newcommand{\Poi}{\mbox{Poi}}
\newcommand{\Student}{{\cal T}}
\newcommand{\student}{{\cal T}}
\newcommand{\Wishart}{\mbox{Wi}}
\newcommand{\Wi}{\mbox{Wi}}
\newcommand{\unif}{\mbox{U}}
\newcommand{\etr}{\mbox{etr}}

\newcommand{\softmax}{\calS}
\newcommand{\soft}{\mbox{soft}}
\newcommand{\cond}{\mbox{cond}}
\newcommand{\sign}{\mbox{sign}}
\newcommand{\sgn}{\mbox{sgn}}
\newcommand{\iid}{\mbox{iid}}
\newcommand{\mle}{\mbox{mle}}
\newcommand{\myiff}{\mbox{iff}}
\newcommand{\pd}{\mbox{pd}}
\newcommand{\pdf}{\mbox{pdf }}
\newcommand{\cdf}{\mbox{cdf}}
\newcommand{\pmf}{\mbox{pmf}}
\newcommand{\wrt}{\mbox{wrt}}
\newcommand{\matlab}{{\sc MATLAB}}
\newcommand{\NETLAB}{{\sc NETLAB}}
\newcommand{\MLABA}{\mbox{PMTK}}
\newcommand{\BLT}{\mbox{PMTK}}
\newcommand{\PMTK}{\mbox{PMTK}}
\newcommand{\mywp}{\mbox{wp}}

\newcommand{\KLpq}[2]{\mathrm{KL}\left[{#1}\|{#2}\right]}
\newcommand{\KL}{\mbox{KL}}
\newcommand{\MI}{\mathbb{I}}
\newcommand{\MIxy}[2]{\mathbb{I}\left({#1};{#2}\right)}
\newcommand{\MIxyz}[3]{\mathbb{I}\left({#1};{#2}|{#3}\right)}
\newcommand{\entropy}[1]{\mathbb{H}\left({#1}\right)}
\newcommand{\entropypq}[2]{\mathbb{H}\left({#1}, {#2}\right)}


\newcommand{\vvec}{\mbox{vec}}
\newcommand{\kron}{\otimes}
\newcommand{\dof}{\mbox{dof}}
%\newcommand{\E}{E}
\newcommand{\E}{\mathbb{E}}
\newcommand{\energy}{E}
\newcommand{\expectAngle}[1]{\langle #1 \rangle}
%\newcommand{\expect}[1]{\mathbb{E}\left[ {#1} \right]}
\newcommand{\expect}[2]{\mathds{E}_{{#1}} \left[ {#2} \right]}
\newcommand{\expectGiven}[3]{\mathds{E}_{{#1}} \left[ {#2} \mid {#3} \right]}
\newcommand{\Var}{\mbox{Var}}
\newcommand{\VarGiven}[3]{\mbox{Var}_{{#1}}\left[ {#2} \mid {#3}\right]}
%\newcommand{\Var}{\mathbb{V}}
\newcommand{\var}[1]{\mbox{var}\left[{#1}\right]}
\newcommand{\std}[1]{\mbox{std}\left[{#1}\right]}
\newcommand{\varQ}[2]{\mbox{var}_{{#2}}\left[{#1}\right]}
\newcommand{\cov}[1]{\mbox{cov}\left[{#1}\right]}
%\newcommand{\mode}[1]{\mbox{mode}\left[{#1}\right]}
\newcommand{\median}[1]{\mbox{median}\left[{#1}\right]}



\newcommand{\diag}{\mbox{diag}}
\newcommand{\blkdiag}{\mbox{blkdiag}}
\newcommand{\bias}{\mbox{bias}}
\newcommand{\union}{\cup}
\newcommand{\intersect}{\cap}

\newcommand{\size}{\mbox{size}}
\newcommand{\trace}{\mbox{trace}}


\newcommand{\myc}{c}
\newcommand{\myi}{i}
\newcommand{\myj}{j}
\newcommand{\myk}{k}
\newcommand{\myn}{n}
\newcommand{\myq}{q}
\newcommand{\mys}{s}
\newcommand{\myt}{t}


\newcommand{\supp}{\mbox{supp}}


\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calDx}{{\cal D}_x}
\newcommand{\calE}{{\cal E}}
\newcommand{\cale}{{\cal e}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calHX}{{\cal H}_X}
\newcommand{\calHy}{{\cal H}_y}
\newcommand{\calI}{{\cal I}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\caln}{{\cal n}}
\newcommand{\calNP}{{\cal NP}}
\newcommand{\calMp}{\calM^+}
\newcommand{\calMm}{\calM^-}
\newcommand{\calMo}{\calM^o}
\newcommand{\Ctest}{C_*}
\newcommand{\calL}{{\cal L}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calq}{{\cal q}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calSstar}{\calS_*}
\newcommand{\calT}{{\cal T}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calv}{{\cal v}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calY}{{\cal Y}}

\newcommand{\Lone}{$\ell_1$}
\newcommand{\Ltwo}{$\ell_2$}

\newcommand{\mya}{\mbox{a}}
\newcommand{\myat}{\alpha_{t|t-1}}
\newcommand{\score}{\mbox{score}}
\newcommand{\AIC}{\mbox{AIC}}
\newcommand{\BIC}{\mbox{BIC}}
\newcommand{\BICcost}{\mbox{BIC-cost}}
\newcommand{\scoreBIC}{\mbox{score-BIC}}
\newcommand{\scoreBICL}{\mbox{score-BIC-L1}}
\newcommand{\scoreL}{\mbox{score-L1}}

\newcommand{\ecoli}{\mbox{{\it E. coli}}}
\newcommand{\doPearl}{\mbox{do}}
\newcommand{\data}{\calD}
\newcommand{\model}{\calM}
\newcommand{\dataTrain}{\calD_{\mbox{train}}}
\newcommand{\dataTest}{\calD_{\mbox{test}}}
\newcommand{\dataValid}{\calD_{\mbox{valid}}}
\newcommand{\futuredata}{\tilde{\calD}}
\newcommand{\algo}{\calA}
\newcommand{\fitAlgo}{\calF}
\newcommand{\predictAlgo}{\calP}
\newcommand{\err}{\mbox{err}}
\newcommand{\logit}{\mbox{logit}}
\newcommand{\parent}{\mbox{pa}}


%%%%%%%%%%% Hoyt

\newcommand{\conv}[1]{\,\,\,\displaystyle{\operatorname*{\longrightarrow}^{\,_{#1}\,}}\,\,\,}
\newcommand{\dconv}{\conv{D}}
\newcommand{\pconv}{\conv{P}}
\newcommand{\asconv}{\conv{AS}}
\newcommand{\lpconv}[1]{\conv{L^{#1}}}

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{n}


\newcommand{\condSet}{\mathcal{S}}
\newcommand{\condSetC}{\mathcal{\lnot S}}



==> math_commands.tex <==
\newcommand*\diff{\mathrm{d}}
\newcommand*\Image{\mathrm{Im}}
\newcommand*\NN{\smash{\hat{\mathcal{F}}_{\scriptsize\textrm{NN}}}}

\newcommand*\X{\mathcal{X}}
\newcommand*\Z{\mathcal{Z}}
\newcommand*\G{\mathcal{G}}
\newcommand*\D{\mathcal{D}}
\newcommand*\F{\mathcal{F}}
\newcommand*\R{\mathcal{R}}
\newcommand*\TR{\hat{R}}
\newcommand*\Deltab{\bar{\Delta}}
\newcommand*\h{h}
\newcommand*\biasb{\mathrm{bias}}
\newcommand*\varb{\mathrm{var}}
\newcommand*\covb{\mathrm{cov}}
\newcommand*\M{\mathcal{M}}
\newcommand*\B{\mathcal{B}}
\newcommand*\W{\mathcal{W}}
\newcommand*\Loss{\mathcal{L}}
\newcommand*{\Ftr}{\smash{\mathcal{F}_{\scriptsize\textrm{tr}}}}
\newcommand*{\Fts}{\smash{\mathcal{F}_{\scriptsize\textrm{ad}}}}
\newcommand*{\Dtr}{\smash{\mathcal{D}_{\scriptsize\textrm{tr}}}}
\newcommand*{\Dts}{\smash{\mathcal{D}_{\scriptsize\textrm{ad}}}}
\newcommand*{\Etr}{\smash{\mathcal{E}_{\scriptsize\textrm{tr}}}}
\newcommand*{\Ead}{\smash{\mathcal{E}_{\scriptsize\textrm{ad}}}}

\newcommand*{\eg}{e.g.,\@\xspace}
\newcommand*{\versus}{vs.\@\xspace}
\newcommand*{\sut}{s.t.\@\xspace}
\newcommand*{\ie}{i.e.,\@\xspace}
\newcommand*{\iid}{ID\@\xspace}
\newcommand*{\sota}{SoTA\@\xspace}
\newcommand*{\ood}{OOD\@\xspace}
\newcommand*{\metric}{metric}
\newcommand*{\wrt}{w.r.t.\@\xspace}
\newcommand*{\iif}{i.i.f.\@\xspace}
\newcommand*{\aka}{a.k.a.\@\xspace}
\newcommand*{\rhs}{r.h.s.\@\xspace}
\newcommand*{\etc}{etc.\@\xspace}
\newcommand*{\cf}{cf.\@\xspace}
\newcommand*{\resp}{resp.\@\xspace}

\newcommand*\er{\mathrm{er}}
\newcommand*\ess{\operatorname{ess}}

\let\originalleft\left
\let\originalright\right
\renewcommand{\left}{\mathopen{}\mathclose\bgroup\originalleft}
\renewcommand{\right}{\aftergroup\egroup\originalright}

\let\up\textsuperscript
\let\vec\boldsymbol


\newcommand{\defeq}{\mathrel{:\mkern-0.25mu=}}
\newcommand{\eqdef}{\mathrel{=\mkern-0.25mu:}}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}
\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\trifigref#1#2#3#4{figures \ref{#1}, \ref{#2}, and \ref{#3}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\Termref#1{Term~\ref{#1}}
\def\twosecref#1#2{sections \ref{#1} and \ref{#2}}
\def\trisecref#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\appref#1{appendix~\ref{#1}}
\def\Appref#1{Appendix~\ref{#1}}
\def\suppref#1{supp.~\ref{#1}}
\def\Suppref#1{Supp.~\ref{#1}}
\def\eqref#1{eq.~\ref{#1}}
\def\Eqref#1{Eq.~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\Tabref#1{Table~\ref{#1}}
\def\tabref#1{table~\ref{#1}}
\def\twotabref#1#2{tables \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}

\newcommand{\Lp}{\mathcal{L}^\text{prior}}
\newcommand{\Ll}{\mathcal{L}^\text{likeli}}
\newcommand{\Lal}{\Ls^{\text{l}\widehat{\text{ikel}}\text{i}}}

\def\eps{{\varepsilon}}


\def\xopt{{x^{*}}}
\def\Gopt{{G^{*}}}

\def\p{{\textnormal{p}}}
\def\P{{\textnormal{p}}}
\def\Q{{\textnormal{q}}}
\def\q{{\textnormal{q}}}

\def\gTh{{\hat \gT}}
\def\gDh{{\hat \gD}}
\def\gPh{{\hat \gP}}
\newcommand{\tin}[1]{\mbox{\tiny $#1$}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\reps{{\mathcal{E}}}
\def\rtheta{{\Theta}}
\def\rx{{X}}
\def\ry{{Y}}
\def\rz{{Z}}


\def\S{\mathcal{S}}
\def\T{\mathcal{T}}
\def\X{\mathcal{X}}
\def\Y{\mathcal{Y}}
\def\U{\mathcal{U}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}
\def\rvtheta{{\bm{\theta}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmx{{\mathbf{x}}}
\def\rmy{{\mathbf{y}}}
\def\rmz{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}
\def\valpha{{\bm{\alpha}}}
\def\vtheta{{\bm{\theta}}}
\def\vdelta{{\bm{\delta}}}
\def\vDelta{{\bm{\Delta}}}
\def\vmu{{\bm{\mu}}}
\def\vphi{{\bm{\phi}}}
\def\vSigma{{\bm{\Sigma}}}
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\E{{\mathcal{E}}}
\def\mBeta{{\bm{\beta}}}
\def\mTheta{{\bm{\theta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}

\def\tx{{\tens{x}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gGh{{\hat\gG}}
\def\gFh{{\hat\gF}}


\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathcal{X}}}
\def\sY{{\mathcal{Y}}}
\def\sZ{{\mathcal{Z}}}
\def\sTheta{{\bm{\Theta}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}
\newcommand{\dd}{\mathrm{d}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\KL}{$\mathrm{KL}$\@\xspace}
\newcommand{\Kl}{\mathrm{KL}}
\newcommand{\Esp}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\slerp}{\mathrm{slerp}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\Span}{\mathrm{Span}}
\newcommand{\card}{\mathrm{card}}


\newcommand{\KLD}[2]{D_{\mathrm{KL}} \left( \left. \left. #1 \right|\right| #2 \right) }
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}



\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\newcommand{\acc}{\mathrm{Acc}}
\newcommand{\1}{\mathds{1}}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> section-7-eval-orig.tex <==

\section{Olmo 3 Evaluation Suite}
\label{sec:eval-suite}

We evaluate \olmothree with three sets of tasks: a \textbf{Base Easy} for making small-scale data decisions, a \textbf{Base Main} suite for our large models in the pre-train and mid-train stages, and a \textbf{Chat} suite for instruct models.

All task suites are publicly available at \texttt{\href{https://github.com/allenai/olmes/tree/new-configs\#olmo-3-eval-suite}{github.com/allenai/olmes\#olmo-3-eval-suite}}.

\subsection{Base Model Evaluation}

The \olmothree base evaluation suite is built starting with the \olmotoo iteration of OLMES \citep{olmo20242olmo2furious,olmes}: we expand the number of benchmarks from 11 tasks to 43 tasks, prioritizing math and code tasks. As both the number and scope of capabilities are larger, it becomes increasingly important to ensure the quality of our evaluation signal. 
We introduce three new innovations to validate the quality of the \olmothree base suite: 
(1) clustering tasks by capability,
(2) tracking the noise of each evalution task, and
(3) a separate task suite for small-scale models by identifying jumps in task performance.

\paragraph{Expanding OLMES tasks.} We expanded our evaluation to target specific capabilities: new QA tasks focusing on science knowledge (SciQ, QASPER, SciRIFF), medical/lab knowledge (ProtocolQA, DBQA, MedMCQA, MedQA), math tasks (GSM Symbolic, Minerva MATH) and coding tasks (DS 1000, BigCodeBench, Deepseek LeetCode\footnote{We use `Deepseek LeetCode' to refer to the 180 LeetCode problems used during development in \citet{guo2024deepseek}}, MultiPL-E HumanEval, MultiPL-E MBPP). We use MultiPL-E to evaluate our multilingual code execution, limited to six core programming languages. Additionally, we track fill-in-the-middle (FIM) performance using HumanEval with the three settings from \citet{bavarian2022efficient}: single-line infilling, multi-line infilling and random span infilling.

We support code execution in Python, C++, Java, JavaScript, PHP, Rust and Shell using AWS Lambda functions to grade instances in parallel, isolated environments of up to 50K generations simultaneously. In total, our environments graded 17.2 million generated code samples during \olmothree development, with up to 1.5K simultaneously. To ensure reproducibility, we release a lightweight Docker library for code execution without AWS infrastructure\footnote{Our code execution environments are publicly available at \texttt{\href{https://github.com/allenai/olmes-docker}{github.com/allenai/olmes-docker}}.}.

\davidh{UltraChat Masked PPL, WildChat Masked PPL (when did these get used?)}


Additionally, \olmotoo only tracked math and code capabilities after mid-training, as small models exhibit random-chance pass@1 performance on math and code tasks \citep{wei2022emergent}. Our base easy suite tracks perplexity over human-written math and code solutions \citep{huang2024compression}, which allows us to broadens the scope of capabilities we track during pre-training.

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/base_eval/clustering_dendrogram}
    \caption{
    Visualization of the task clustering procedure. The clustering method iteratively merges tasks which rank models similarly, until arriving at a manually defined stop condition. We used this method do identify the 5 clusters used in development. \davidh{TODO: We manually moved some tasks around (e.g. DS1000, CruxEval under code cluster, some basic skills are in wrong place).}
    }
    \label{fig:clustering_dendrogram}
\end{figure}

\paragraph{Clustering Tasks.} To handle the large number of tasks, we cluster similar tasks into macro-averages, and use the averages as our signal for data interventions. We aim for the number of task clusters to match the granularity at which we perform data interventions, and for tasks within each cluster to behave similarly. Our clustering procedure requires a process to determine the similarity of two evaluations -- we do this by collecting a large pool of scores from 70 external, open-weight models resulting in a set of 23K evaluation benchmark results. 

Using our dataset of evaluation results, we assume that two benchmarks evaluate similar constructs if they rank models similarly. We perform hierarchical clustering using Ward's variance-minimization \citep{ward1963hierarchical}, which iteratively merges evaluation scores to minimize the variance of scores between benchmarks within a cluster. Figure \ref{fig:clustering_dendrogram} shows the result of the clustering procedure, where we manually select a threshold to balance the amount and granularity of clusters. Importantly, we do not use the exact result of the clustering procedure -- we manually move a few tasks to ensure the format of the task is the same within each cluster (e.g. tasks requiring code execution all occur in the same cluster). The resulting task clusters are: \textbf{STEM QA}, \textbf{Non-STEM QA}, \textbf{GenQA}, \textbf{Math}, \textbf{Code} and \textbf{Code FIM} (fill-in-the-middle), as grouped in Table \ref{tab:task-details}.

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/base_eval/snr_midtrain}
    \caption{
    Training curves of midtraining on canonical language model benchmarks (top), and our proposed base main task suites (bottom) for QA, Math and Code.
    We used the signal-to-noise ratio of early mid-training runs to make decisions about aggregating evaluation scores. Our resulting task averages had a better signal-to-noise ratio than individual benchmarks.
    } 
    \label{fig:snr-midtrain}
\end{figure}

\paragraph{Signal-to-noise Analysis.}
When reporting a macro-average, we aimed to exclude tasks from each cluster that were too noisy to be helpful for development. We use calculate the signal-to-noise ratio of each benchmark following the method from \citet{heineman2025signalnoiseframeworkreducing}, where we evaluate the final 50 checkpoints of \olmotoo 13B training, and 10 external base models trained at roughly the same compute scale ($4\cdot10^{23}$ FLOPs). From our findings, we transition from using 1K instance subsets to full evaluation sets when available. We remove some benchmarks from our evaluation suite entirely, particularly binary benchmarks such as BoolQ \citep{clark-etal-2019-boolq}, as we found that models usually oscillate between predicting the majority and minority class.

We repeat the same analysis for mid-training, instead using intermediate checkpoints from 5 preliminary pre-training runs. One important finding was to separate some benchmarks from the macro-average, like CruxEval \citep{gu2024cruxeval}, which measures a relevant and unique capability (code input/output prediction), but would introduce too much noise into the macro-average. We show an example of the SNR of three individual benchmarks compared to the base main task averages across intermediate checkpoints during midtraining in Figure \ref{fig:snr-midtrain}.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/base_eval/scaling_analysis}
    \caption{
    Scaling analysis for the \olmothree base evaluation suite. At the largest scale used to run from-scratch data ablations (grey line, a 1B model trained to 100B tokens), our `base main' evaluation suite is too difficult to show improvement (top figures). Instead, we introduce a `base easy' suite to compare models at small scales (bottom figures).
    } 
    \label{fig:scaling-analysis}
\end{figure}

\paragraph{Scaling Analysis.} Some evaluation benchmarks are too difficult to show signal when training models at small scales \citep{wei2022emergent}, and other benchmarks no longer provide useful signal as the performance `saturates' or approaches the labeling error of the benchmark \citep{vendrow2025large}. 
\citet{ruan2024observational} shows that the reported training compute of open-weight can be used to observe the compute scales at which behaviors `emerge', which we use here to validate the scaling behavior of our benchmarks.
When designing the \olmothree evaluation suite, we evaluated on the suite of \olmotoo scaling law models from \citet{bhagia2024establishingtaskscalinglaws} to understand the scaling behavior in the low-compute regime, and open-weight models to understand scaling behavior in the high-compute regime.
Figure~\ref{fig:scaling-analysis} shows the scaling behavior for our resulting base main benchmarks. For each task family, the easy task suite showed signal at the small data ablation scale, and the main task suites were not saturated at the large scale, leaving headroom for data experiments in midtraining.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/base_eval/easy_to_main}
    \caption{
    Relationship between bits-per-byte using the `Easy' suite and final metrics using the `Main' evaluation suite. We use the `Easy' suite to make decisions at a small scale, which corresponds to an improvement at the large scale.
    \davidh{Add a rank correlation claim -- because BPB corresponds to improved task perf at larger scales, it is OK to use at small scales to make decisions.}
    } 
    \label{fig:easy-to-main}
\end{figure}

\input{tables/base_eval/eval_config}
\input{tables/base_eval/easy_eval_config}

\subsubsection{Base Evaluation Suites}

Using the analysis tools described in the previous section, we construct two evaluation suite for decision making in pre-training: the \textbf{Base Easy} suite for small-scale data decisions and the \textbf{Base Main} suite for in-loop evaluation and mid-training data decisions. We kept the number of in-context examples and generation arguments consistent within each family of tasks, when possible\footnote{We perform all evaluation using vLLM. To prevent performance discrepancies between versions, we pin to \texttt{v0.9.0.1} for evaluation during development, and pin to \texttt{v0.11.0} for all evaluation in the final report.}.

Table \ref{tab:task-details} describes the task configuration and metrics for the \olmothree base evaluation suite.

\paragraph{Base Easy Suite.}
\citet{schaeffer2023emergent} noticed while many tasks appear emergent, often proxy metrics (e.g. perplexity-based metrics) can be used to indicate model performance is improving before we exit the noise floor.
Previous work has highlighted the use of continuous metrics for making modeling decisions for pre-training \citep{huang2024compression,magnusson2025datadecidepredictbestpretraining}. 
In particular, that continuous metrics show a smoother improvement during training, and are less likely to result in a false ranking due to noise \citep{heineman2025signalnoiseframeworkreducing}.
We measure bits-per-byte over tasks from the base main suite which have gold answers, calculated as the negative log-likelihood of the answer divided by the number of UTF-8 bytes in the answer string, as described in \citet{gao2020pile}.
For multiple-choice BPB, we simply use the correct answer as the continuation.
For math BPB, we use the provided human-written solutions from Minerva MATH \citep{lewkowycz2022solving}. 
For code BPB, we use the gold `canontical' solution as provided in HumanEval and MBPP \citep{chen2021codex,austin2021program}. 
For BPB over non-Python coding tasks, MultiPL-E did not release gold solutions \citep{cassano2022multipl}, so we generate silver continuations for 16 languages using \texttt{o4-mini-medium}\footnote{We release this generation set at \texttt{\href{https://huggingface.co/datasets/allenai/multilingual_mbpp}{huggingface.co/datasets/allenai/multilingual\_mbpp}}}. Figure \ref{fig:scaling-analysis} shows the scaling behavior of the three base easy task clusters, where we see signal even at very small (190M parameter) model sizes.

One important property of the base eval suite is that a ranking of two small models on the base easy suite agrees with their ranking on the downstream base main suite. We validate this by measuring rank correlation between the easy and main task suites, as pictured in Figure \ref{fig:easy-to-main}. \davidh{Add: Compared to measuring C4 validation loss, our easy task suite has substantially higher rank correlation at the large scale.}

\begin{wrapfigure}{r}{0.45\linewidth}
    \centering
    \vspace{-10pt}
    \includegraphics[width=\linewidth]{figures/base_eval/temperature_sweep}
    \caption{To select generation arguments for base evaluation, we run a temperature and top-p sweep across 5 models. We use a reasonable configuration such that we can calculate both pass@1 and pass@k using the results of a single evaluation job.}
    \label{fig:temperature-sweep}
    \vspace{-10pt}
\end{wrapfigure}

\paragraph{Base Main suite} As a result of the clustering procedure, the base main suite tracks 6 task groups: MCQA STEM, MCQA Non-STEM, Gen, Math, Code, Code FIM. Unlike \olmotoo, we are tracking generative math and code tasks at pre-training. We chose to evaluate pass@k with the largest number of samples such that each task could evaluate on \olmotoo 7B on 1 H100 in under 30 minutes, in order to ensure the eval speed is not bottlenecked by any particular task. For tasks with a large enough $n$, we set $k=16$ to match the GRPO group size, which we observed to act as an empirical upper-bound on the possible improvement from RL training. To decide on the the temperature and top-p, we ran a sweep and evaluated 5 models (\olmotoo 7B, 13B; Qwen 2.5 7B, 13B; Qwen 3 8B; \citealp{qwen2.5,qwen3}) to find an adequate configuration setting for high scores on both pass@1 and pass@k. Results are shown in Figure \ref{fig:temperature-sweep}, and we select temperature and top-p of 0.6 for all base math and code evaluation.

\paragraph{Base Chat suite} During mid-training, we refashion the chat eval suite (\S\ref{sec:chat-eval-suite}) for use evaluating base models, which served as a reference as to whether we expect our model to perform well after the adaptation pipeline. To do this, we used a standard, simple chat template (\texttt{Question: \{text\}\textbackslash nAnswer:}) across all base models (both \olmothree and baseline models) and we included stop tokens to prevent degenerate responses. We also excluded tasks which required an API-based judge (AlpacaEval, SimpleQA) due to cost. In practice, we noticed that most of the disagreements between the base main and base chat evaluation suites were due to noise, so we mainly used the base suite for making decisions.

\paragraph{Base Long-Context suite} During the long-context extension phase, we evaluate long-context capability using RULER as our primary development signal. As a complementary held-out set, we also use HELMET, noting that the HELMET \emph{Recall} task directly implements several RULER evaluations (specifically \texttt{ruler_niah_mk_2}, \texttt{ruler_niah_mk_3}, and \texttt{ruler_niah_mv}). Because we evaluate only base models at this stage, we disable chat templates within HELMET to ensure consistent scoring across models. For HELMET tasks requiring an LLM-as-a-judge, we use its default judge configuration (\texttt{gpt-4o-2024-05-13}). Taken together, RULER guides most model-selection decisions during long-context development, with HELMET providing an additional check on generalization.

\paragraph{Base Held-out suite} We targeted one held-out evaluation task to match each family of capability: MMLU Pro for QA \citep{wang2024mmlu}, LBPP for code \citep{matton-etal-2024-leakage}, Deepmind Math for math \citep{saxton2019analysing}, and BigBench Hard to measure broad coverage across unseen task types \citep{suzgun2022challenging}. 


\subsubsection{New Evaluation Benchmarks}
\label{sec:new-evaluation-benchmarks}

\paragraph{Basic Skills} We developed a new benchmark, \textsc{BasicSkills}, to measure whether core capabilities are being acquired during pretraining. \textsc{BasicSkills} consists of 6 subtasks: basic arithmetic, string manipulation, simple coding, elementary logical reasoning, basic common sense, and simple pattern recognition. Each task isolates a single skill using a self-contained context that requires no external knowledge or additional information and can be completed through natural text continuation without relying on instruction-following abilities.

\paragraph{Gen2MC} One takeaway from \olmotoo development was a sensitivity to task format. The clustering procedure furhter confirmed this, finding that generative scores rank models similarly as rank choice (RC) QA tasks, disagreeing with ranking of single-token multiple choice (MC) QA tasks (see Figure \ref{fig:clustering_dendrogram}). In particular, the short-form generative QA tasks (GenQA in Table \ref{tab:evals_overview}) evaluate by comparing a generated answer to a bank of plausible answers, but these answer banks are often not complete, leading to false negatives. To address this, we introduce the \textbf{Gen2MC} benchmarks, which were constructed by taking the original question/answer pairs and generating incorrect multiple-choice distractor answers using a strong LLM. For each set of generated distractors, we manually review a set of 200 sample questions from the validation set before generating the full dataset. We create Gen2MC tasks for DROP, Jeopardy, NaturalQs, SQuAD, CoQA using GPT-4o for generating distractors, and fall-back to GPT-4.1 in cases where output parsing failed.






\subsection{Post-trained Model Evaluation}
\label{sec:posttrain_eval}
We evaluated post-trained \olmothree models on a suite of benchmarks targeting knowledge-recall, reasoning, math, coding, tool use, chat, instruction following, and safety. 
We expand upon the evaluation suite we used in \cite{olmo20242olmo2furious} and \cite{lambert2024tulu3} to include ... \jm{new and more difficult evaluations in domains we evaluated before, and evaluations in new domains entirely (eg puzzle data). we also use (DEEPSEEK SETTINGS), and we report the average of 3 eval runs to account for variance (deeper dive into variance?)}
\hamish{Add a few things: guiding philosophy of always being zero-shot, stripping thinking traces from answer so that only the final answer is judged for things like AlpacaEval.}

\jm{TODO: Simplify intro, I stole a bunch from above for 9.2.1}

\input{tables/instruct/eval_config_posttrain}

\subsubsection{Chat Evaluation Suite}
\label{sec:chat-eval-suite}
\todo{Jacob}

\paragraph{Improvements to the \olmotoo Evaluation Suite} 
We made substantial \jm{pick diff word} improvements to the evaluation suite we used when building \olmotoo when designing the \olmothree evaluation suite. We removed TruthfulQA~\CITE{} as it did not provide much useful signal when training, and we removed DROP~\CITE{} due to frequent formatting issues that did not correlate with model capabilities. We additionally updated AlpacaEval 2 Lenth Controlled (LC)~\CITE{} to use GPT-4.1 (\CITE{}?) as a judge instead of the original GPT-4-Turbo (\CITE{}?) both to increase the reliability of the evaluation and to save $\sim$90\% of inference costs. 

Table \ref{tab:task-details-chat} describes the task configurations and metrics for the \olmothree chat evaluation suite.

\paragraph{New Evaluations} We also expanded our evaluation suite to include new and more difficult evaluations in domains we already measured, and evaluations in domains we had not previously trained for. We added SimpleQA~\CITE{}, GPQA~\CITE{}, ZebraLogic~\CITE{}, AGI Eval English~\CITE{} (previously an unseen evaluation for both \olmotoo and \tulu), OMEGA~\CITE{}, AIME~\CITE{}, MBPP Plus~\CITE{}, and LiveCodeBench~\CITE{}. We also added BFCL~\CITE{}, LitQA~\CITE{}, and SimpleQA with Tools~\CITE{}, detailed in depth in Section~\jm{TOOL USE SECTION}, and \jm{SAFETY EVALS} in Section~\jm{SAFETY SECTION}.

\jm{I don't love just listing evals, but I'm not sure if we want to go in depth on like, what category each are in, why we added each, etc? Maybe we could point towards category, like "we added knowledge evals x y z, coding evals x y z, ...} \davidh{Agree! Maybe we could have a table for the post-train evals (similar to Tab. \ref{tab:task-details}), and only talk about what was new in the text? (changing AE judge, temp/top-p, averaging across runs, tool use)}

\paragraph{Designing a Single Reasoning-Ready Evaluation Suite}
An important criteria for us while designing our evaluation suite was to make sure we could use the same evaluations for both \olmothreethinking and \olmothreethinking. We first decided to only use generative evaluations, rather than \jm{?}. We also set the sampling temperature to 0.6 as in the DeepSeek R1 report~\CITE{}, rather than 0.0 as in \olmotoo, because both thinking and instruct models benefit from higher temperatures \CITE{} \jm{or say thinking are degen with t=0}. To account for the variance introduced by making our evaluations inherently less deterministic, we report the average of 3 runs for all models. For QA tasks (e.g. BBH, MMLU), we created a unified set of `Olmo 3' regexes for answer extraction.

\todo{Jacob}

\jm{Need to note how we accounted for variance?}

\subsubsection{Evaluating tool use}

We evaluated the tool use capabilities of \olmothreeinstruct in terms of \textit{function calling} and \textit{task completion} accuracies using different benchmarks. We used the Berkeley Function Calling Leaderboard (BFCLv3)~\citep{patil2025bfcl} to evaluate function calling accuracy. This benchmark focuses on models' ability to choose the relevant functions and the right values for their arguments to accomplish a given task in settings that require one or more interactions with simulated users and environments. We evaluated the task completion accuracy of \olmothreeinstruct in comparison with similar models when they are deployed as agents with access to tools served via Model Context Protocol (MCP) servers. Particularly, we used the Asta Scientific Corpus (ASC) tool~\pradeep{cite AstaBench} that serves eight functions for accessing scientific literature, and the Serper API which provides Google search tool and web browsing functionalities. We evaluated the models on LitQA2~\citep{skarlinski2024language} to evaluate models' usage of the ASC tool and SimpleQA~\citep{wei2024measuring} for search and browsing tools.


We use the official Gorilla repository for BFCLv3 evaluations. For LitQA2 and SimpleQA, we implement a basic function calling agent using OpenAI's Agent SDK. This agent uses the tools provided by the relevant MCP server, and interacts with the environment by iteratively making function calls and processing the outputs of executing them to solve the given tasks.
For LitQA2 and SimpleQA, We also measure model performance when deployed in a \textit{No-Tools} setting, in which we provide no tools to the agents and they are expected to solve the tasks entirely from the models' parametric knowledge. We use a zero-shot evaluation for all these benchmarks. We sample from models at temperature 0 and for LitQA2 and SimpleQA, allow the agents at most 10 turns to finish each task. We run each evaluation three times and report the average accuracy.









\subsubsection{Safety evaluation}

\begin{table}[]
    \centering
\begin{tabular}{llrrllllllll}
            & HarmBench & DAN & XSTest & WG-Test & WJb-Test & JbT & Toxigen & StrRej & WMDP & BBQ & \textbf{Average} \\
    Model 1 &           &                                   &                            &                &                    &                  &         &              &      &     &                  \\
    Model 2 &           &                                   &                            &                &                    &                  &         &              &      &     &                  \\
    Model 3 &           &                                   &                            &                &                    &                  &         &              &      &     &
    \end{tabular}
    \label{tab:safety-evals}
    \caption{\maarten{this is probably how the table will look!}}
\end{table}


The safety evaluations that were tested upon during training runs were the same set from OLMo2 \citep{olmo2024olmo2} and Tulu3 \citep{lambert2024tulu3}. 
In addition to the development safety evaluations \ref{ssec:evals-seen-safety}, we also evaluate our models on four new safety evaluations, chosen due to their prevalence in recent LLM safety evaluations \citep{kaiyom2024helmsafety,gemini2.5,claude4,gpt5,aegisLLM,lambert2024tulu3}.

\paragraph{Development safety evaluations} %
include HarmBench~\citep{mazeika2024harmbench}, DoAnythingNow~\citep[DAN;][]{shen2024anything}, XSTest \citep{rottger2023xstest}, WildGuard-Test \citep{han2024wildguard}, WildJailbreak-Test \citep{jiang2024wildteaming}, and TrustLLM-JailbreakTrigger \citep{huang2024trustllm}. More details about these evaluations can be found in the Appendix~\ref{sec:appendix_safety_evals}.

\paragraph{Unseen safety evaluations}%
that we added were Toxigen~\citep{toxigen}, StrongReject~\citep{strongreject}, Weapons of Mass Destruction Proxy~\citep[WMDP;][]{wmdp}, and Bias Benchmark for QA~\citep[BBQ;][]{parrish-etal-2022-bbq}. More details about these evaluations can be found in Appendix~\ref{sec:appendix_safety_evals}.

\paragraph{Averaging and reported metrics} Safety and accuracy scores are aggregated according to benchmark protocol, with all reported metrics normalized such that higher values are better (1 indicates perfect safety performance).
Specifically, we report the average of: \textit{refusal accuracy}, i.e., inverted ASR (Attack Success Rate), for DoAnythingNow, Harmbench, Wildguard, TrustLLM-JailbreakTrigger, Toxigen, and StrongReject; \textit{accuracy} for XSTest and BBQ; the average of inverted ASR for Wildjailbreak (harmful) and ASR for Wildjailbreak (benign); and inverted accuracy (i.e., error rate) for WMDP.

\subsection{Benchmark Decontamination}
\subsubsection{Pretraining and midtraining data}
\pradeep{One difference between base and post-training decontamination is that it seems like in base you filtered the evaluation data, whereas in post-train we filtered the training data. I am guessing filtering the training data is not really feasible in pretrain and midtrain? It is worth pointing that out if so.}

\ianm{[WIP]} Contamination of evaluation instances in training can cause overestimation of performance, so we investigate and remove contamination from the benchmarks we use. As memorization occurs most strongly near the end of training \citep{Magar2022DataCF, Bordt2024HowMC}, we focus our efforts to applying decontamination at midtraining time. 

Table~\ref{tab:decon_overestimation} shows the performance difference when applying midtraining decontamination or not. DROP shows heavy performance overestimation without decontamination but only when used as a generative rather than MC task. Code Gen pass @ 16 also shows performance overestimation across most subtasks but this is not the case for when not using pass @ 1.

Table~\ref{tab:base_evals_contam_perf_and_counts} shows base evaluation benchmarks sorted by performance overestimation (contaminated - decontaminated performance). We also show the percentage of benchmark instances that are contaminated. Note that high \% contamination does not always lead to performance overestimation if tasks are saturated or near trivial performance.

\begin{table}[]
    \begin{scriptsize}
    \centering
    \begin{tabular}{lrrrr}
    \toprule
    Eval. & \% Contam & Perf. Overest. & Contam Perf & Decon. Perf. \\
    \midrule
    Drop & 66.87 & 13.99 & 58.93 & 72.92 \\
    GSM-Symb & 0.00 & 5.54 & 52.07 & 57.61 \\
    Codex Humaneval @ 16 & 7.07 & 3.54 & 68.81 & 72.35 \\
    DeepSeek LeetCode @ 16 & 47.22 & 3.24 & 0.00 & 3.24 \\
    Drop MC & 2.05 & 2.39 & 63.92 & 66.31 \\
    MultiPL-E MBPP & 0.01 & 1.86 & 37.70 & 39.56 \\
    Squad & 83.24 & 1.70 & 92.17 & 93.87 \\
    GSM8K & 84.99 & 1.61 & 78.49 & 80.10 \\
    Coqa & 2.44 & 1.36 & 72.77 & 74.13 \\
    MultiPL-E HumanEval @ 16 & 5.36 & 1.32 & 53.90 & 55.22 \\
    Winogrande & 0.32 & 1.11 & 85.10 & 86.21 \\
    Jeopardy MC & 0.04 & 1.05 & 86.41 & 87.46 \\
    MBPP @ 16 & 1.14 & 1.00 & 59.67 & 60.67 \\
    DS1000 & 0.00 & 0.88 & 19.50 & 20.38 \\
    BigCodeBench & 0.00 & 0.75 & 35.79 & 36.54 \\
    Medqa En MC & 1.98 & 0.71 & 42.18 & 42.89 \\
    Lambada & 10.15 & 0.56 & 70.00 & 70.56 \\
    Sciq MC & 6.43 & 0.39 & 92.82 & 93.21 \\
    FiM & 7.07 & 0.38 & 33.77 & 34.15 \\
    Naturalqs MC & 0.03 & 0.35 & 68.93 & 69.28 \\
    ARC MC & 13.26 & 0.34 & 89.32 & 89.66 \\
    Socialiqa MC & 0.01 & 0.34 & 80.26 & 80.60 \\
    Medmcqa MC & 0.46 & 0.14 & 49.61 & 49.75 \\
    MMLU MC & 5.30 & 0.09 & 66.88 & 66.97 \\
    Squad MC & 0.57 & 0.05 & 97.30 & 97.35 \\
    Basic & 0.02 & 0.02 & 89.90 & 89.92 \\
    Hellaswag & 2.75 & 0.01 & 78.66 & 78.67 \\
    Naturalqs & 0.38 & -0.22 & 32.71 & 32.49 \\
    MBPP & 1.14 & -0.25 & 49.18 & 48.93 \\
    MultiPL-E MBPP @ 16 & 0.01 & -0.28 & 61.61 & 61.33 \\
    Coqa MC & 1.81 & -0.43 & 93.76 & 93.33 \\
    DeepSeek LeetCode & 47.22 & -0.56 & 0.56 & 0.00 \\
    MultiPL-E HumanEval & 5.36 & -0.95 & 29.54 & 28.59 \\
    Codex Humaneval & 7.07 & -1.03 & 50.46 & 49.43 \\
    CSQA MC & 1.80 & -1.08 & 76.68 & 75.60 \\
    Jeopardy & 5.37 & -1.41 & 61.79 & 60.38 \\
    Piqa MC & 3.28 & -1.77 & 81.47 & 79.70 \\
    Minerva & 45.17 & -1.95 & 44.09 & 42.14 \\
    \bottomrule
    \end{tabular}
    \caption{Base evaluation benchmarks sorted by performance overestimation (contaminated - decontaminated performance). We also show the percentage of benchmark instances that are contaminated. Note that high \% contamination does not always lead to performance overestimation if tasks are saturated or near trivial performance. }
    \label{tab:base_evals_contam_perf_and_counts}
    \end{scriptsize}
\end{table}

\ianm{TODO: describe decon method} https://github.com/allenai/decon/blob/main/doc/simple.md

\subsubsection{Post-training data} \label{sec:posttraining_decontam}
We followed the recommended settings from the Tulu 3 Decontamination Procedure and toolkit \cite{lambert2024tulu3} to filter out the portions of the post-training data that matched the evaluation sets. We used n-gram matching with 8-grams and an overlap threshold of 0.5 (i.e., at least 50\% of the n-grams in the test instance match a training instance) for filtering. We developed additional heuristics to mitigate false-positives: 1) We ignored matches of task-irrelevant chunks of text, e.g. common generic phrases, with the irrelevance determined per task based on manual inspection; 2) Particularly in math datasets, we ignored matches of n-grams where most of the tokens are of length 1 (typically math symbols). \pradeep{Saumya, is this a good summary? Also are these heuristics implemented in the decontamination code? If so, it is worth pointing out that we updated it.}


\begin{table}[t]
\centering
\small
\begin{tabularx}{\textwidth}{@{}l@{\hspace{1em}}X@{}}
\toprule

\textbf{Aggregated} &
\makebox[\linewidth][c]{%
\begin{tabular}{@{}ccccccc@{}}
\textbf{MCQA (STEM)} & \textbf{MCQA (Non-STEM)} & \textbf{Gen} & \textbf{Math} & \textbf{Code Gen} & \textbf{Code Gen pass@16} & \textbf{Code FIM} \\
\midrule
\cellcolor[HTML]{FAFDFC}-0.26 & \cellcolor[HTML]{FCFDFD}-0.08 & \cellcolor[HTML]{FAE3E1}1.90 & \cellcolor[HTML]{F0F9F5}-1.73 & \cellcolor[HTML]{FCFDFC}-0.10 & \cellcolor[HTML]{FAE5E3}1.76 & \cellcolor[HTML]{FAFDFB}-0.38 \\
\end{tabular}
}
\\[1.25ex]

\textbf{Gen} &
\makebox[\linewidth][c]{%
\begin{tabular}{@{}ccccccccc@{}}
\textbf{Hellaswag} & \textbf{Winogrande} & \textbf{Lambada} & \textbf{Basic RC} & \textbf{DROP} & \textbf{Jeopardy} & \textbf{Naturalqs} & \textbf{Squad} & \textbf{COQA} \\
\midrule
\cellcolor[HTML]{D0ECDE}0.01 & \cellcolor[HTML]{FEFAFA}1.11 & \cellcolor[HTML]{FFFFFF}0.56 & \cellcolor[HTML]{D0ECDE}0.02 & \cellcolor[HTML]{E67C73}13.99 & \cellcolor[HTML]{57BB8A}-1.41 & \cellcolor[HTML]{BCE4D0}-0.22 & \cellcolor[HTML]{FDF4F4}1.70 & \cellcolor[HTML]{FEF8F7}1.36 \\
\end{tabular}
}
\\[1.25ex]

\textbf{Code Gen @16} &
\makebox[\linewidth][c]{%
\begin{tabular}{@{}ccccc@{}}
\textbf{Deepseek Leetcode} & \textbf{Codex Humaneval} & \textbf{MBPP} & \textbf{MultiPL-E HumanEval} & \textbf{MultiPL-E MBPP} \\
\midrule
\cellcolor[HTML]{FBE9E8}3.24 & \cellcolor[HTML]{FBE6E5}3.54 & \cellcolor[HTML]{FBFDFC}1.00 & \cellcolor[HTML]{FFFDFD}1.32 & \cellcolor[HTML]{A4DABF}-0.28 \\
\end{tabular}
}
\\

\bottomrule
\end{tabularx}

\caption{Performance differences in aggregated base development benchmarks between final midtrained model
with and without decontamination. We expand Gen and Code Gen Pass @ 16 to show where overestimation specifically occurs. In Gen overestimation of contaminated DROP performance stands out, while overestimation is present in most Code Gen @ 16 evaluations.}
\label{tab:decon_overestimation}
\end{table}

